HIT: A Hierarchically Fused Deep Attention Network for Robust Code-mixed Language Representation

Understanding linguistics and morphology of resource-scarce code-mixed texts remains a key challenge in text processing. Although word embedding comes in handy to support downstream tasks for low-resource languages, there are plenty of scopes in improving the quality of language representation particularly for code-mixed languages. In this paper, we propose HIT, a robust representation learning method for code-mixed texts. HIT is a hierarchical transformer-based framework that captures the semantic relationship among words and hierarchically learns the sentence-level semantics using a fused attention mechanism. HIT incorporates two attention modules, a multi-headed self-attention and an outer product attention module, and computes their weighted sum to obtain the attention weights. Our evaluation of HIT on one European (Spanish) and five Indic (Hindi, Bengali, Tamil, Telugu, and Malayalam) languages across four NLP tasks on eleven datasets suggests significant performance improvement against various state-of-the-art systems. We further show the adaptability of learned representation across tasks in a transfer learning setup (with and without fine-tuning).

==> tab-dataset-stats.tex <==
\begin{table*}
    \centering
    \begin{tabular}{c r r r}
    \hline
         Sentiment Label & Train & Dev & Test \\
         \hline
         Neutral & 1,562 & 89 & 94 \\
         Positive & 1,087 & 205 & 209 \\
         Negative & 454 & 94 & 85 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Hindi-English sentiment dataset}
    \label{tab:hi_sentiment_data}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c r r r}
        \hline
         Sentiment Label & Train & Dev & Test \\
         \hline
         Positive & 2,022 & 224 & 565 \\
         unknown\_state & 1,344 & 161 & 398 \\
         not-malayalam & 647 & 60 & 177\\
         Negative & 549 & 51 & 138 \\
         Mixed\_feelings & 289 & 44 & 70 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Malayalam-English sentiment dataset}
    \label{tab:ma_sentiment_data}
\end{table*}

\begin{table*}
    %\centering
    \begin{tabular}{c r r r}
        \hline
         Sentiment Label & Train & Dev & Test \\
         \hline
         Positive & 7,627 & 857 & 2,075 \\
         Negative & 1,448 & 165 & 424 \\
         Mixed\_feelings & 1,283 & 141 & 377 \\
         unknown\_state & 609 & 68 & 173 \\
         not-Tamil & 368 & 29 & 100\\
            \hline
    \end{tabular}
    \caption{Label distribution for Tamil-English sentiment dataset}
    \label{tab:ta_sentiment_data}
\end{table*}

\begin{table*}
    \centering
    \begin{tabular}{c r r r}
    \hline
         Sentiment Label & Train & Dev & Test \\
         \hline
         Positive & 6,848 & 1,073 & 1,073 \\
         Neutral & 3,363 & 517 & 517 \\
         Negative & 1,983 & 305 & 305 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Spanish-English sentiment dataset}
    \label{tab:sp_sentiment_data}
\end{table*}

\begin{table}
    \centering
    \begin{tabular}{c r r r}
    \hline
         PoS Label & Train & Dev & Test \\
         \hline
        N\_NN & 2,896  & 817   & 668 \\
    V\_VM & 1,503  & 388   & 302 \\
    RD\_PUNC & 1,387  & 451   & 394 \\
    N\_NNP & 1,010  & 288   & 224 \\
    PSP   & 756   & 287   & 226 \\
    PR\_PRP & 708   & 268   & 210 \\
    JJ    & 552   & 160   & 152 \\
    RB\_AMN & 276   & 74    & 52 \\
    CC    & 255   & 66    & 50 \\
    QT\_QTF & 232   & 46    & 53 \\
    DM\_DMD & 231   & 23    & 25 \\
    RP\_RPD & 206   & 49    & 45 \\
    RD\_RDF & 174   & 57    & 64 \\
    V\_VAUX & 150   & 51    & 42 \\
    DT    & 140   & 37    & 28 \\
    PR\_PRQ & 118   & 20    & 19 \\
    \#    & 92    & 52    & 39 \\
    RP\_NEG & 89    & 40    & 38 \\
    E     & 85    & 28    & 30 \\
    \$    & 84    & 18    & 14 \\
    RB\_ALC & 82    & 26    & 18 \\
    N\_NNV & 61    & 28    & 24 \\
    PR\_PRL & 53    & 16    & 30 \\
    N\_NST & 51    & 23    & 13 \\
    RP\_INJ & 48    & 10    & 6 \\
    RD\_SYM & 42    & 18    & 13 \\
    DM\_DMR & 26    & 9     & 14 \\
    RP\_INTF & 26    & 15    & 7 \\
    PR\_PRF & 24    & 8     & 7 \\
    QT\_QTO & 16    & 3     & 1 \\
    QT\_QTC & 5     & 5     & 2 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Bengali-English PoS dataset}
    \label{tab:ben_pos_data}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{c r r r}
    \hline
         PoS Label & Train & Dev & Test \\
         \hline
    X     & 6,108  & 747   & 780 \\
    VERB  & 4,792  & 586   & 595 \\
    NOUN  & 3,950  & 582   & 620 \\
    ADP   & 2,336  & 303   & 315 \\
    PROPN & 2,250  & 439   & 400 \\
    ADJ   & 1,247  & 151   & 153 \\
    PART  & 1,163  & 216   & 198 \\
    PRON  & 1,163  & 165   & 174 \\
    DET   & 914   & 120   & 130 \\
    ADV   & 802   & 91    & 111 \\
    CONJ  & 640   & 92    & 91 \\
    PART\_NEG & 369   & 52    & 57 \\
    PRON\_WH & 329   & 42    & 52 \\
    NUM   & 311   & 44    & 25 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Hindi-English PoS dataset}
    \label{tab:hin_pos_data}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{c r r r}
    \hline
         PoS Label & Train & Dev & Test \\
         \hline
N\_NN & 5,284  & 403   & 374 \\
    N\_NNP & 3,279  & 280   & 287 \\
    RD\_RDF & 2,796  & 98    & 82 \\
    RD\_PUNC & 2,532  & 215   & 221 \\
    V\_VM & 2,227  & 185   & 148 \\
    JJ    & 1,206  & 106   & 102 \\
    PSP   & 988   & 92    & 76 \\
    PR\_PRP & 757   & 69    & 37 \\
    RP\_INJ & 527   & 24    & 29 \\
    DT    & 479   & 42    & 41 \\
    RB\_AMN & 478   & 33    & 29 \\
    CC    & 285   & 31    & 18 \\
    \$    & 261   & 25    & 26 \\
    U     & 247   & 1     & 11 \\
    E     & 245   & 66    & 51 \\
    \#    & 218   & 10    & 11 \\
    N\_NNV & 90    & 9     & 7 \\
    \&    & 88    & 13    & 6 \\
    PR\_PRQ & 83    & 5     & 1 \\
    V\_VAUX & 81    & 21    & 16 \\
    RD\_PUNC" & 80    & 1     & 5 \\
    ~     & 67    & 6     & 7 \\
    QT\_QTF & 45    & 11    & 5 \\
    RD\_UNK & 45    & 2     & 1 \\
    DM\_DMD & 38    & 5     & 3 \\
    RP\_RPD & 21    & 3     & 4 \\
    RB\_ALC & 9     & 3     & 2 \\

            \hline
    \end{tabular}
    \caption{Label distribution for Telegu-English PoS dataset}
    \label{tab:telugu_pos_data}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{c r r r}
    \hline
         PoS Label & Train & Dev & Test \\
         \hline
    VERB  & 35,297 & 5,459  & 5c,459 \\
    PUNCT & 33,922 & 5,310  & 5,310 \\
    PRON  & 33,243 & 5,180  & 5,180 \\
    NOUN  & 19,416 & 2,935  & 2,935 \\
    DET   & 15,361 & 2,310  & 2,310 \\
    ADV   & 14,570 & 2,177  & 2,177 \\
    ADP   & 12,515 & 1,949  & 1,949 \\
    INTJ  & 10,435 & 1,602  & 1,602 \\
    CONJ  & 7,684  & 1,173  & 1,173 \\
    ADJ   & 7,257  & 1,082  & 1,082 \\
    AUX   & 7,178  & 1,082  & 1,082 \\
    SCONJ & 6,840  & 1,039  & 1,039 \\
    PART  & 4,576  & 725   & 725 \\
    PROPN & 4,502  & 688   & 688 \\
    NUM   & 2,634  & 382   & 382 \\
    UNK   & 1,624  & 250   & 250 \\
    X     & 14    & 2     & 2 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Spanish-English PoS dataset}
    \label{tab:spanish_pos_data}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{c r r r}
    \hline
         NER Label & Train & Dev & Test \\
         \hline
    O     & 25,283 & 3,239  & 3,056 \\
    B-PERSON & 1,317  & 161   & 158 \\
    B-PLACE & 616   & 74    & 58 \\
    I-PERSON & 574   & 74    & 71 \\
    B-ORGANISATION & 300   & 33    & 45 \\
    I-PLACE & 146   & 7     & 13 \\
    I-ORGANISATION & 85    & 8     & 17 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Hindi-English NER dataset}
    \label{tab:hindi_ner_data}
\end{table}

\begin{table}
    \centering
    \begin{tabular}{c r r r}
    \hline
         NER Label & Train & Dev & Test \\
         \hline
        O     & 392,704 & 119,209 & 119,209 \\
    B-PER & 3,140  & 940   & 940 \\
    B-LOC & 1,683  & 511   & 511 \\
    I-PER & 986   & 283   & 283 \\
    B-PROD & 906   & 256   & 256 \\
    I-LOC & 896   & 256   & 256 \\
    I-TITLE & 764   & 216   & 216 \\
    B-TITLE & 540   & 157   & 157 \\
    B-ORG & 506   & 154   & 154 \\
    B-GROUP & 417   & 118   & 118 \\
    B-TIME & 364   & 108   & 108 \\
    I-ORG & 333   & 91    & 91 \\
    I-PROD & 316   & 91    & 91 \\
    I-EVENT & 195   & 57    & 57 \\
    B-OTHER & 187   & 65    & 65 \\
    I-GROUP & 181   & 53    & 53 \\
    I-TIME & 139   & 38    & 38 \\
    B-EVENT & 138   & 46    & 46 \\
    I-OTHER & 33    & 7     & 7 \\
            \hline
    \end{tabular}
    \caption{Label distribution for Spanish-English NER dataset}
    \label{tab:spanish_ner_data}
\end{table}

==> tab-parameters.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|l|c||c}
         {\bf Tasks} & {\bf Lang} & {\bf Model} & {\bf \# Params(M)} & {\bf Train Time(s/ep)}\\
          
          \hline
         \multirow{6}{*}{\rotatebox{90}{\bf Sentiment}} & \multirow{6}{*}{\bf Hi-En} & CS-ELMo & 2.9 & 18 \\
          & & HAN & 2.7 & 14\\
          & & Subword-LSTM & 2.1 & 7\\
          & & BiLSTM & 2.8 & 12 \\
          & & ML-BERT & 179.2 & 172 \\
          \cline{3-4}
          & & \cellcolor{blue!10} {\bf \name} & \cellcolor{blue!10} 2.7 & \cellcolor{blue!10} 13  \\
          \hline
          \multirow{5}{*}{\rotatebox{90}{\bf POS}} & \multirow{5}{*}{\bf Hi-En} & CS-ELMo & 2.4 & \\
          & & HAN & 1.4 &\\
          %& & Subword-LSTM & 2.1\\
          & & BiLSTM-CRF & 1.5 &\\
          & & ML-BERT & 177.9 &\\
          \cline{3-4}
          & & \cellcolor{blue!10} {\bf \name} & \cellcolor{blue!10} 1.4 & \cellcolor{blue!10} \\
          \hline
    \end{tabular}}
    \caption{Parameters per Model for various tasks. %Datasets marked with * do not contain separate train-dev-test split. For * datasets we use 10-fold cross validation.
    }
    \label{tab:parameters}
\end{table}

==> tab-sentiment-feature.tex <==
\begin{table}
\centering
%%\vspace*{-0.21cm}
\resizebox{\columnwidth}{!}
{
\begin{tabular}{l|c|c|c||c}
\hline
 \textbf{Model} & {\bf Hi-En} & {\bf Ta-En} & {\bf Ma-En} & {\bf Sp-En} \\
\hline
HIT & 0.871 & 0.364 & 0.507 & 0.392 \\
HIT + Features & \textbf{0.913} & \textbf{0.473} & \textbf{0.651} & \textbf{0.445} \\
\hline
\end{tabular}}%
\caption{Advantages of using Statistical features with HIT on Sentiment Classification Tasks. Best scores are highlighted in bold.}
  \label{tab:allresultssentimentfeatures}%
\end{table}%
